Concurrent object-oriented development with behavioral design patterns

The development of concurrent applications is challenging because of the complexity of concurrent designs and the hazards of concurrent programming. Architectural modeling using the Unified Modeling Language (UML) can support the development process, but the problem of mapping the model to a concurrent implementation remains. This paper addresses this problem by defining a scheme to map concurrent UML designs to a concurrent object-oriented program. Using the COMET method for the architectural design of concurrent object-oriented systems, each component and connector is annotated with a stereotype indicating its behavioral design pattern. For each of these patterns, a reference implementation is provided using SCOOP, a concurrent object-oriented programming model. We evaluate this development process using a case study of an ATM system, obtaining a fully functional implementation based on the systematic mapping of the individual patterns. Given the strong execution guarantees of the SCOOP model, which is free of data races by construction, this development method eliminates a source of intricate concurrent programming errors.

==> discussion.tex <==

\section{Discussion}
\label{sec:discussion}

This section discusses the lessons learned from implementing the COMET
design patterns, in particular with regard to the choice of 
implementation language.

% \subsection{SCOOP design considerations}
% \label{sec:design-considerations}

% One of the benefits that SCOOP provides is a protection against data
% races by design.  The concurrency model and the type system together
% provide this guarantee: independent processors contain their own data,
% and the type system protects the access to that data.  This
% encapsulation of concurrency maps directly to the behavioral patterns.

% In turn, it lowers the number of concepts involved in the design as
% opposed to an implementation that used threads as the low-level
% concurrency model.

% With any use of concurrency, one must be careful to avoid
% deadlock situations.
% Consider a queue with reply: 
% the sender puts a non-separate message into the
% conduit and waits on a reply from the receiver.  After, the receiver
% issues a call on the message, thus the receiver must wait on the
% sender to become free to answer the message call.  Since the sender is
% waiting on the receiver, and vice-versa, there is a deadlock
% situation.
% We found that the messages that are
% sent should either be of an expanded type (\eif{INTEGER}, \eif{REAL},
% etc.) or reside on a distinct processor from the sender to
% eliminate the threat of deadlock.

% There is also a question of whether to use inheritance or regular
% objects to form the endpoints of the connectors.  Using regular
% objects is likely the better choice, as they offer a more flexible
% solution: if constructed by a factory, only the factory need know
% about the underlying conduit for the endpoints.  A solution which uses
% inheritance would have to pass this conduit during the construction of
% the object which inherits the endpoint.

\subsection{Expressivity of concurrency models}
\label{sec:expressivity-models}

Especially since the advent of multicore processors, there has been
much research interest in defining novel concurrency models. When
evaluating such models, attention must also be given to their
expressivity, i.e.\ which types of concurrency problems a model can
handle. One of the important open questions in this respect is
\emph{how} expressivity can be evaluated.

Behavioral patterns could be used to provide a framework to evaluate
the expressivity in a uniform way: namely by determining which
patterns a language can implement, and whether there are any
complications with implementing individual patterns.  In the case of
SCOOP we can report that it can successfully implement all but one of
COMET's suggested behavioral stereotypes (not ``multi-read
entities''). The inability to implement multiple readers stems
directly from the message-passing nature of the SCOOP model: since
there is no shared memory, not only concurrent writers but also
concurrent readers are excluded. This is an important practical
limitation (shared with all message-passing models, which lend
themselves better to distributed computation), and is correctly
detected by trying to implement the COMET patterns.

\subsection {Comparing SCOOP and Java}
\label{sec:compare-scoop-java}
An alternative implementation of the ATM system is also
available for Java.
While similar, the two implementations differ in several ways.
Firstly, the Java system must rely on programmer competence to 
ensure data race freedom;
this is a manual and generally difficult task.
As all data is potentially shared in Java programs,
one must determine which data is read/written by
more than one thread, and protect it accordingly.
SCOOP does not require such manual tasks,
as it ensures data race freedom by construction.
This happens when data is sent from one component to another:
in SCOOP it is impossible to access the data from both the
sending and receiving side, while in Java this is possible.

Secondly, the concurrent data structures used in both examples
(such as the concurrent queues used in the connectors)
require different implementation styles due to the language.
Although Java contains first-class support for concurrent programming
through the inclusion of monitors for every object,
implementing a concurrent queue still requires a measure of caution.
For example, implementing a condition variable requires the
identification of the condition,
waiting on the object that embodies the condition and 
rechecking the condition manually,
and having a corresponding signal in another routine that
is fired only when the condition is true.
All of these actions have the possibility to introduce an error.
In SCOOP, these manual tasks 
(wait, notification, and condition identification) 
are rolled into a single concept: the wait-condition.
Signaling and waiting happen automatically, reducing the problem
to only ensuring that the correct precondition is used.


% \subsection {SCOOP design considerations}
% \label{sec:design-considerations}

% One of the benefits that SCOOP provides is a protection against data
% races by design.  The concurrency model and the type system together
% provide this guarantee: independent processors contain their own data,
% and the type system protects the access to that data.  This
% encapsulation of concurrency maps directly to the behavioral patterns.

% % In turn, it lowers the number of concepts involved in the design as
% % opposed to an implementation that used threads as the low-level
% % concurrency model.

% With any use of concurrency, one must be careful to avoid
% deadlock situations.
% Consider a queue with reply: 
% the sender puts a non-separate message into the
% conduit and waits on a reply from the receiver.  After, the receiver
% issues a call on the message, thus the receiver must wait on the
% sender to become free to answer the message call.  Since the sender is
% waiting on the receiver, and vice-versa, there is a deadlock
% situation.
% We found that the messages that are
% sent should either be of an expanded type (\eif{INTEGER}, \eif{REAL},
% etc.) or reside on a distinct processor from the sender to
% eliminate the threat of deadlock.

% There is also a question of whether to use inheritance or regular
% objects to form the endpoints of the connectors.  Using regular
% objects is likely the better choice, as they offer a more flexible
% solution: if constructed by a factory, only the factory need know
% about the underlying conduit for the endpoints.  A solution which uses
% inheritance would have to pass this conduit during the construction of
% the object which inherits the endpoint.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

